Lossless Acceleration of Large Language Models with Hierarchical Drafting based on Temporal Locality in Speculative Decoding

Accelerating inference in Large Language Models (LLMs) is critical for real-time interactions, as they have been widely incorporated into real-world services. Speculative decoding, a fully algorithmic solution, has gained attention for improving inference speed by drafting and verifying tokens, thereby generating multiple tokens in a single forward pass. However, current drafting strategies usually require significant fine-tuning or have inconsistent performance across tasks. To address these challenges, we propose Hierarchy Drafting (HD), a novel lossless drafting approach that organizes various token sources into multiple databases in a hierarchical framework based on temporal locality. In the drafting step, HD sequentially accesses multiple databases to obtain draft tokens from the highest to the lowest locality, ensuring consistent acceleration across diverse tasks and minimizing drafting latency. Our experiments on Spec-Bench using LLMs with 7B and 13B parameters demonstrate that HD outperforms existing database drafting methods, achieving robust inference speedups across model sizes, tasks, and temperatures.

==> figure/ablation.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.99\columnwidth]{figure/DB.jpg}
\vspace{-.8em}
\caption{\small Ablation study with bars showing the ratios of draft failures, successes, and draft \& verify successes, and the line indicating the acceptance ratio.}
\label{fig:ablation}
% \vspace{-2.0em}
\end{figure}

==> figure/ablation_and_token_coverage.tex <==
\begin{figure*}[t!]
\centering
\begin{minipage}{0.75\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figure/DB.jpg}
\end{minipage}
\hfill
\begin{minipage}{0.24\textwidth}
    \centering
    \includegraphics[width=0.99\textwidth]{figure/overlap.jpg}
\end{minipage}
\vspace{-.8em}
v\caption{\small Breakdown study of the exploited database in HD using Llama-2-7b-chat on Spec-Bench. (Left) Ablation study with bars showing the ratios of draft failures, successes, and draft \& verify successes, and the line indicating the acceptance ratio. (Right) Venn diagram of accepted tokens using a single database.}
\label{fig:ablation_and_token_coverage}
\vspace{-1.5em}
\end{figure*}

==> figure/latency_and_acceptance.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.95\columnwidth]{figure/latency_and_acceptance.jpg}
\vspace{-.8em}
\caption{\small Drafting accuracy (\%) and latency (ms) for tuning-free drafting methods of speculative decoding in greedy sampling with Vicuna-7b on Spec-Bench~\cite{Spec_Survey}. The value next to the marker means the acceleration ratio compared to autoregressive decoding.}
\label{fig:latency_and_acceptance}
\vspace{-2.0em}
\end{figure}


==> figure/spec_bench.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.95\columnwidth]{figure/spec_bench.jpg}
\vspace{-.8em}
\caption{\small Acceleration results on each category of Spec-Bench with tuning-free drafting methods.}
\label{fig:spec_bench}
% \vspace{-1.5em}
\end{figure}

==> figure/spec_bench_and_latency_vs_acceptance.tex <==
\begin{figure}[t!]

        \centering
        \includegraphics[width=\columnwidth]{figure/spec_bench.jpg}
    \caption{\small Acceleration results on each category of Spec-Bench with database drafting methods.}
\label{fig:spec_bench_and_latency_vs_acceptance}
\end{figure}

==> figure/step_len.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.95\columnwidth]{figure/step_len.jpg}
\vspace{-.8em}
\caption{\small .}
\label{fig:step_len}
% \vspace{-1.5em}
\end{figure}

==> table/DB_details.tex <==
\begin{table}[t]
    \caption{\small } \label{tab:DB_details}
    \vspace{-1mm}
    \centering
    \renewcommand{\arraystretch}{1}
\resizebox{.99\columnwidth}{!}{
    \begin{tabular}{l  c c }
    \toprule
       \textbf{DB} & \textbf{Database Scale} & \textbf{Drafting Latency}  \\ \midrule
       \(\mathcal{D}_c\) & 519 \(\pm\) 423 & 0.31 \(\pm\) 0.06 ms \\
       \(\mathcal{D}_m\) & 100K & 0.02 ms \\ 
       \(\mathcal{D}_s\) & 200M & 2.86 \(\pm\) 6.43 ms \\ \bottomrule
    \end{tabular}
} 
% \vspace{-1.5em}
\end{table}

==> table/draft_hit_and_verify_success.tex <==
\begin{table}[t]
    \caption{\small } \label{tab}
    \vspace{-1mm}
    \centering
    \renewcommand{\arraystretch}{1}
\resizebox{.99\columnwidth}{!}{
    \begin{tabular}{l  c c c}
    \toprule
       \textbf{Method} & \textbf{Database Scale} & \textbf{Drafting Latency}  & \textbf{Token/Sec} \\ \midrule
       \textbf{PLD}~\cite{PLD} & 519 \(\pm\) 423 & 0.31 \(\pm\) 0.06 ms& 74.51 \(\pm\) 23.09 \\
       \textbf{LADE}~\cite{LAD} & 354 \(\pm\) 258 & < 0.01 ms & 66.34 \(\pm\) 14.09\\ 
       \textbf{REST}~\cite{REST} & 200M & 2.86 \(\pm\) 6.43 ms & 66.04 \(\pm\) 14.72\\ \bottomrule
    \end{tabular}
} 
\vspace{-1.5em}
\end{table}
